Unifying Correspondence, Pose and NeRF for Pose-Free Novel View Synthesis from Stereo Pairs

This work delves into the task of pose-free novel view synthesis from stereo pairs, a challenging and pioneering task in 3D vision. Our innovative framework, unlike any before, seamlessly integrates 2D correspondence matching, camera pose estimation, and NeRF rendering, fostering a synergistic enhancement of these tasks. We achieve this through designing an architecture that utilizes a shared representation, which serves as a foundation for enhanced 3D geometry understanding. Capitalizing on the inherent interplay between the tasks, our unified framework is trained end-to-end with the proposed training strategy to improve overall model accuracy. Through extensive evaluations across diverse indoor and outdoor scenes from two real-world datasets, we demonstrate that our approach achieves substantial improvement over previous methodologies, especially in scenarios characterized by extreme viewpoint changes and the absence of accurate camera poses.

==> sec/tables/ablation.tex <==
\begin{wraptable}{r}{0.55\textwidth}
% \begin{table*}[!t]
\centering
\vspace{-10pt}
    \caption{\textbf{Ablation study for \ours.} We conduct ablation study by gradually adding components to the cost aggregation baseline.}
    \vspace{-10pt}
    \label{tab:ablation}
\resizebox{\linewidth}{!}{
\begin{tabular}{ll|ccccc}
        \toprule
        &Components & PSNR & LPIPS & SSIM & Rot. & Trans. & 
         \\ 
        \midrule\midrule
        \textbf{(I)} & Feature Agg. & 3.8 & 10.9 & 19.1 & 53.5 & 96.2 \\    
        
        \textbf{(II)} & Cost Agg.  & 14.7& \underline{23.2}& 35.3& 60.3& \underline{96.7}&78.9\\
        %\textbf{(III)} &\textcolor{gray}{\textbf{(II)}} + \textcolor{gray}{Transformer} & 9.9& 15.1& 28.5& 57.0& 96.2& 76.4\\
        \textbf{(III)} &\textbf{(II)} + Spatial agg.  & 14.9& 23.1& 35.9& 60.3& \underline{96.7}&79.5\\
        \textbf{(IV)} &\textbf{(II)} + Class agg.  & 14.7& 21.5& 36.6& 60.6& 95.5&80.5\\
        \textbf{(V)} &\textbf{(II)} + Spatial and Class agg. & \underline{15.5}& \underline{23.2}& \underline{37.0}& \underline{62.3}& \underline{96.7}&\underline{81.3}\\
        \textbf{(VI)} &\textbf{(V)} + Embedding guidance  & \textbf{16.0} & \textbf{23.8}& \textbf{37.9}& \textbf{63.3}& \textbf{97.0}&\textbf{82.5}\\
        \bottomrule
\end{tabular}
}
% \end{table*}
    \vspace{-10pt}
\end{wraptable}

